TRUER: Test-Time Reward Correction Using an Error-Aware Rectifier for Reinforcement Learning

Test-time reinforcement learning enables language models to adapt using rewards derived from their own answers. However, majority voting can reinforce incorrect solutions even when correct alternatives are available. Our training audit shows that false positives (incorrect responses receiving positive rewards) dominate reward errors. We focus on a practical regime where ground-truth rewards are difficult to obtain at scale, while a limited labeled source set is available. We introduce TRUER, a framework that uses limited supervision to train a reward rectifier that distinguishes correctness from consensus. To achieve this goal, we train the rectifier with an emphasis on incorrect majorities and correct minorities, targeting cases where consensus and correctness disagree. After that, we freeze the rectifier and use it to correct rewards during subsequent test-time adaptation. By improving reward accuracy and thereby model performance, TRUER consistently outperforms naive TTRL in both metrics across all evaluated configurations.

==> tables/all_steps_rows.tex <==
15 & TTRL & 73.51 & 58.46 & 72.43 & 81.89 & 92.70 \\
15 & Rank1-only & 72.70 & 57.90 & 72.33 & 82.16 & 92.43 \\
15 & TRUER & 72.43 & 59.33 & 73.07 & 80.27 & 91.89 \\
15 & Oracle & 72.16 & 58.56 & 72.49 & 81.62 & 92.16 \\
\midrule
30 & TTRL & 72.43 & 65.49 & 76.99 & 84.05 & 92.97 \\
30 & Rank1-only & 72.97 & 65.46 & 76.77 & 82.70 & 93.24 \\
30 & TRUER & 74.59 & 66.10 & 77.16 & 84.05 & 93.78 \\
30 & Oracle & 74.59 & 66.08 & 77.35 & 83.51 & 93.24 \\
\midrule
45 & TTRL & 75.68 & 67.76 & 78.22 & 84.05 & 92.70 \\
45 & Rank1-only & 76.22 & 68.52 & 78.75 & 84.05 & 93.24 \\
45 & TRUER & 75.68 & 68.51 & 78.87 & 84.59 & 93.51 \\
45 & Oracle & 76.76 & 68.55 & 79.07 & 84.32 & 93.24 \\
\midrule
60 & TTRL & 77.30 & 68.74 & 78.81 & 83.24 & 92.43 \\
60 & Rank1-only & 75.68 & 69.21 & 79.04 & 83.78 & 93.51 \\
60 & TRUER & 75.95 & 69.76 & 79.44 & 84.59 & 93.24 \\
60 & Oracle & 78.11 & 70.11 & 79.99 & 85.95 & 92.70 \\
\midrule
75 & TTRL & 78.92 & 69.15 & 78.68 & 82.70 & 92.16 \\
75 & Rank1-only & 77.57 & 69.97 & 79.27 & 83.51 & 93.78 \\
75 & TRUER & 75.95 & 70.27 & 79.73 & 84.59 & 93.24 \\
75 & Oracle & 78.65 & 70.46 & 80.03 & 85.95 & 92.97 \\
\midrule
90 & TTRL & 76.22 & 69.62 & 79.33 & 83.24 & 92.97 \\
90 & Rank1-only & 76.22 & 70.04 & 79.51 & 83.78 & 94.32 \\
90 & TRUER & 76.49 & 70.46 & 79.76 & 84.86 & 91.89 \\
90 & Oracle & 77.30 & 70.87 & 80.32 & 85.41 & 93.24 \\


==> tables/margin_filter_rows.tex <==
TTRL (no filter) & 56,596 & 4,012 & 2,557 & 93.38 & 100.0 & 0.0 \\
Vote margin $\delta{=}8$ & 54,133 & 1,299 & 1,815 & 97.66 & 95.6 & 67.6 \\
Vote margin $\delta{=}10$ & 53,143 & 1,014 & 1,714 & 98.13 & 93.9 & 74.7 \\
Vote margin $\delta{=}12$ & 52,110 & 928 & 1,636 & 98.25 & 92.1 & 76.9 \\
Absolute support $\geq 24$ & 43,692 & 496 & 1,179 & 98.88 & 77.2 & 87.6 \\
TRUER (ours) & 55,400 & 1,081 & 2,105 & 98.09 & 97.9 & 73.1 \\


==> tables/rank1_intervals_rows.tex <==
TRUER $-$ rank1 & Greedy & +0.27 & [-2.43, +2.97] \\
TRUER $-$ rank1 & Pass@1 & +0.42 & [-0.37, +1.28] \\
TRUER $-$ rank1 & Pass@2 & +0.25 & [-0.54, +1.11] \\
TRUER $-$ rank1 & Majority@32 & +1.08 & [-1.35, +3.51] \\
TRUER $-$ rank1 & Pass@32 & -2.43 & [-4.32, -0.81] \\
\midrule
Rank1 $-$ TTRL & Greedy & +0.00 & [-2.70, +2.70] \\
Rank1 $-$ TTRL & Pass@1 & +0.42 & [-0.37, +1.17] \\
Rank1 $-$ TTRL & Pass@2 & +0.17 & [-0.68, +1.00] \\
Rank1 $-$ TTRL & Majority@32 & +0.54 & [-1.89, +2.97] \\
Rank1 $-$ TTRL & Pass@32 & +1.35 & [-0.54, +3.24] \\

